From Evidence to Effect: Authority Semantics and Runtime Infrastructure for Stateful Agents

Stateful agents reuse artifacts after producing executions and permissions change. We formalize authority-sufficient observations and durable effects bound to execution and material identities. WTB implements this interface through runtime adapters, shared evidence, and transactional publication/recovery. Six study families separate the mechanism from its integration. Raw and typed evidence both solve 32/32 authority cases, with model-dependent planning effects. Fixed-intent enforcement blocks six unsafe proposals and executes 12 eligible authorized intents. Complete controls match WTB's capability. Paid integration yields 176/210 accepted benchmark-source stages, including 19/30 publication stages, recovery on 8/8 primary SWE repositories, and the most complete continuous trajectories on each of three source tasks. The findings connect authority information, effect admission, and infrastructure reuse in stateful agents.

==> tables/adoption_by_source.tex <==
TeamBench & WTB & 60/70 & 7.8092 & 0.1302 \\
TeamBench & Git/Auth & 42/70 & 10.4596 & 0.2490 \\
TeamBench & CONTINUITY & 34/70 & 11.3921 & 0.3351 \\
TeamBench & MasDrift & 34/70 & 11.5695 & 0.3403 \\
BulkPR-Bench & WTB & 58/70 & 7.8240 & 0.1349 \\
BulkPR-Bench & Git/Auth & 39/70 & 10.0774 & 0.2584 \\
BulkPR-Bench & CONTINUITY & 39/70 & 11.3779 & 0.2917 \\
BulkPR-Bench & MasDrift & 35/70 & 11.6088 & 0.3317 \\
Terminal-Bench & WTB & 58/70 & 7.4805 & 0.1290 \\
Terminal-Bench & Git/Auth & 40/70 & 8.4698 & 0.2117 \\
Terminal-Bench & CONTINUITY & 35/70 & 9.1306 & 0.2609 \\
Terminal-Bench & MasDrift & 34/70 & 10.5746 & 0.3110 \\


==> tables/adoption_cohorts_main.tex <==
Controlled fixture & 51/70 (7.47) & 39/70 (10.23) & 37/70 (11.57) & 39/70 (11.73) \\
TeamBench & 60/70 (7.81) & 42/70 (10.46) & 34/70 (11.39) & 34/70 (11.57) \\
BulkPR-Bench & 58/70 (7.82) & 39/70 (10.08) & 39/70 (11.38) & 35/70 (11.61) \\
Terminal-Bench & 58/70 (7.48) & 40/70 (8.47) & 35/70 (9.13) & 34/70 (10.57) \\


==> tables/adoption_stages.tex <==
E0 & 26/30 & 6/30 & 9/30 & 9/30 \\
E1 & 19/30 & 7/30 & 0/30 & 3/30 \\
E2 & 22/30 & 9/30 & 4/30 & 1/30 \\
E3 & 25/30 & 28/30 & 29/30 & 24/30 \\
E4 & 29/30 & 12/30 & 12/30 & 14/30 \\
E5 & 30/30 & 30/30 & 27/30 & 23/30 \\
E6 & 25/30 & 29/30 & 27/30 & 29/30 \\


==> tables/adoption_task1.tex <==
WTB & 8 & 7 & 8 & 8 & 9 & 10 & 10 \\
Git/Auth & 2 & 2 & 4 & 10 & 4 & 10 & 10 \\
CONTINUITY & 3 & 0 & 1 & 10 & 2 & 9 & 9 \\
MasDrift & 5 & 0 & 0 & 8 & 4 & 7 & 10 \\


==> tables/adoption_task2.tex <==
WTB & 8 & 7 & 6 & 9 & 10 & 10 & 8 \\
Git/Auth & 2 & 2 & 3 & 8 & 5 & 10 & 9 \\
CONTINUITY & 4 & 0 & 1 & 10 & 6 & 8 & 10 \\
MasDrift & 2 & 2 & 1 & 7 & 6 & 7 & 10 \\


==> tables/adoption_task3.tex <==
WTB & 10 & 5 & 8 & 8 & 10 & 10 & 7 \\
Git/Auth & 2 & 3 & 2 & 10 & 3 & 10 & 10 \\
CONTINUITY & 2 & 0 & 2 & 9 & 4 & 10 & 8 \\
MasDrift & 2 & 1 & 0 & 9 & 4 & 9 & 9 \\


==> tables/authority_main.tex <==
G0 & 0/32 & 0/32 \\
C0 & 0/32 & 0/32 \\
R0 & 32/32 & 31/32 \\
W0 & 32/32 & 32/32 \\


==> tables/code_changes.tex <==
TeamBench & WTB & 5 & 134.6 & 553.4 & 111.4 \\
TeamBench & Git/Auth & 2 & 250.0 & 525.5 & 119.5 \\
TeamBench & CONTINUITY & 0 & -- & -- & -- \\
TeamBench & MasDrift & 2 & 219.0 & 616.5 & 122.5 \\
BulkPR-Bench & WTB & 6 & 135.3 & 608.3 & 110.8 \\
BulkPR-Bench & Git/Auth & 3 & 280.0 & 515.7 & 112.3 \\
BulkPR-Bench & CONTINUITY & 1 & 208.0 & 764.0 & 96.0 \\
BulkPR-Bench & MasDrift & 2 & 294.0 & 440.5 & 123.0 \\
Terminal-Bench & WTB & 6 & 115.7 & 553.5 & 108.5 \\
Terminal-Bench & Git/Auth & 0 & -- & -- & -- \\
Terminal-Bench & CONTINUITY & 2 & 302.0 & 877.5 & 129.5 \\
Terminal-Bench & MasDrift & 2 & 288.5 & 795.5 & 130.5 \\


==> tables/common_costs.tex <==
TeamBench & Git/Auth & 5 & 0.2277 & 0.4985 & 54.3\% \\
BulkPR-Bench & Git/Auth & 0 & 0.3237 & 0.3275 & 1.2\% \\
BulkPR-Bench & Git/Auth & 4 & 0.2621 & 0.3794 & 30.9\% \\
BulkPR-Bench & Git/Auth & 9 & 0.2202 & 0.3293 & 33.1\% \\
BulkPR-Bench & CONTINUITY & 9 & 0.2202 & 0.3362 & 34.5\% \\
Terminal-Bench & MasDrift & 9 & 0.2737 & 0.4714 & 41.9\% \\


==> tables/continuous.tex <==
TeamBench & WTB & 5/10 & 1.9719 & 0.3944 \\
TeamBench & Git/Auth & 2/10 & 2.5753 & 1.2876 \\
TeamBench & CONTINUITY & 0/10 & 2.5949 & -- \\
TeamBench & MasDrift & 2/9 & 2.7355 & 1.3677 \\
BulkPR-Bench & WTB & 6/10 & 2.3017 & 0.3836 \\
BulkPR-Bench & Git/Auth & 3/9 & 1.6399 & 0.5466 \\
BulkPR-Bench & CONTINUITY & 1/10 & 2.6173 & 2.6173 \\
BulkPR-Bench & MasDrift & 2/10 & 2.8625 & 1.4312 \\
Terminal-Bench & WTB & 6/9 & 2.1263 & 0.3544 \\
Terminal-Bench & Git/Auth & 0/10 & 1.7891 & -- \\
Terminal-Bench & CONTINUITY & 2/10 & 1.5764 & 0.7882 \\
Terminal-Bench & MasDrift & 2/10 & 2.8251 & 1.4125 \\


==> tables/continuous_compact.tex <==
TeamBench & 5/10 (6/8) & 2/10 (3/10) & 0/10 (3/7) & 2/9 (2/8) \\
BulkPR-Bench & 6/10 (8/8) & 3/9 (4/6) & 1/10 (1/9) & 2/10 (2/9) \\
Terminal-Bench & 6/9 (8/9) & 0/10 (3/9) & 2/10 (2/5) & 2/10 (2/9) \\


==> tables/continuous_paired.tex <==
TeamBench & Git/Auth & 10 & 4 & 1 & 1 & 0.3750 & 1.0000 \\
TeamBench & CONTINUITY & 10 & 5 & 0 & 0 & 0.0625 & 0.5000 \\
TeamBench & MasDrift & 9 & 5 & 2 & 0 & 0.4531 & 1.0000 \\
BulkPR-Bench & Git/Auth & 9 & 3 & 0 & 3 & 0.2500 & 1.0000 \\
BulkPR-Bench & CONTINUITY & 10 & 5 & 0 & 1 & 0.0625 & 0.5000 \\
BulkPR-Bench & MasDrift & 10 & 6 & 2 & 0 & 0.2891 & 1.0000 \\
Terminal-Bench & Git/Auth & 9 & 6 & 0 & 0 & 0.0312 & 0.2812 \\
Terminal-Bench & CONTINUITY & 9 & 6 & 1 & 0 & 0.1250 & 0.7500 \\
Terminal-Bench & MasDrift & 9 & 5 & 1 & 1 & 0.2188 & 1.0000 \\


==> tables/continuous_stages.tex <==
TeamBench & WTB & 8/10 & 6/8 & 5/6 & 5/5 \\
TeamBench & Git/Auth & 10/10 & 3/10 & 2/3 & 2/2 \\
TeamBench & CONTINUITY & 7/10 & 3/7 & 1/3 & 0/1 \\
TeamBench & MasDrift & 8/9 & 2/8 & 2/2 & 2/2 \\
BulkPR-Bench & WTB & 8/10 & 8/8 & 7/8 & 6/7 \\
BulkPR-Bench & Git/Auth & 6/9 & 4/6 & 4/4 & 3/4 \\
BulkPR-Bench & CONTINUITY & 9/10 & 1/9 & 1/1 & 1/1 \\
BulkPR-Bench & MasDrift & 9/10 & 2/9 & 2/2 & 2/2 \\
Terminal-Bench & WTB & 9/9 & 8/9 & 8/8 & 6/8 \\
Terminal-Bench & Git/Auth & 9/10 & 3/9 & 2/3 & 0/2 \\
Terminal-Bench & CONTINUITY & 5/10 & 2/5 & 2/2 & 2/2 \\
Terminal-Bench & MasDrift & 9/10 & 2/9 & 2/2 & 2/2 \\


==> tables/e4_failures.tex <==
TeamBench & WTB & 6 & 0 & 1 & 1 & 2 \\
TeamBench & Git/Auth & 3 & 7 & 0 & 0 & 0 \\
TeamBench & CONTINUITY & 3 & 4 & 0 & 0 & 3 \\
TeamBench & MasDrift & 2 & 5 & 1 & 0 & 1 \\
BulkPR-Bench & WTB & 8 & 0 & 0 & 0 & 2 \\
BulkPR-Bench & Git/Auth & 4 & 1 & 1 & 0 & 3 \\
BulkPR-Bench & CONTINUITY & 1 & 8 & 0 & 0 & 1 \\
BulkPR-Bench & MasDrift & 2 & 7 & 0 & 0 & 1 \\
Terminal-Bench & WTB & 8 & 0 & 1 & 0 & 0 \\
Terminal-Bench & Git/Auth & 3 & 5 & 1 & 0 & 1 \\
Terminal-Bench & CONTINUITY & 2 & 1 & 2 & 0 & 5 \\
Terminal-Bench & MasDrift & 2 & 7 & 0 & 0 & 1 \\


==> tables/parity_main.tex <==
Git/Auth & 36/56 & 56/56 \\
CONTINUITY & 44/56 & 56/56 \\
MasDrift & 28/56 & 56/56 \\


==> tables/planning_main.tex <==
GM0 & 12/16 & 5/8 & 7/8 & 2/32 \\
R0 & 9/16 & 8/8 & 1/8 & 2/32 \\
W0 & 6/16 & 0/8 & 6/8 & 11/32 \\


==> tables/runtime_main.tex <==
WTB & 120/120 & 0 & 60/60 \\
Independent SQL guard & 120/120 & 0 & 60/60 \\
CONTINUITY-bound & 120/120 & 0 & 60/60 \\
Remove exact-attempt binding & 108/120 & 12 & 60/60 \\
Remove monotone reconciliation & 102/120 & 6 & 48/60 \\
Remove authority generation & 114/120 & 6 & 60/60 \\
Remove approval consumption & 108/120 & 12 & 48/60 \\
Remove unknown-effect recovery & 114/120 & 0 & 54/60 \\


==> tables/swe_main.tex <==
WTB & 5/8 & 8/8 & 4/8 & 3.1825 & 6.0202 \\
Git/Auth & 1/8 & 1/8 & 0/8 & 3.8082 & 4.9509 \\
CONTINUITY & 2/8 & 1/8 & 0/8 & 4.8002 & 7.1524 \\
MasDrift & 1/8 & 1/8 & 0/8 & 3.4498 & 6.4444 \\

